Machine Intelligence that Understands Visual and Linguistic Information and Interacts with Humans and Environments

Advancements at the intersection of computer vision and natural language processing are crucial for applications like assistive tech, multimedia querying, and robotics. This dissertation proposes novel architectures to improve intelligent agents across three key vision-language tasks: image captioning, visual dialog, and interactive instruction following. First, we address limitations in visual representation for image captioning. Traditional models rely on region-based features from CNN detectors, which lack global context and suffer from high computational overhead. We propose GRIT (Grid and Region-based Image captioning Transformer), a transformer-only architecture. By integrating grid and region features using a DETR-based detector, GRIT enables end-to-end training and out-performs prior methods in both inference accuracy and speed. Second, we tackle visual dialog, which requires multi-turn conversation about an image. The challenge lies in efficiently modeling interactions between multiple inputs (image, question, history). We introduce LTMI (Light-weight Transformer for Many Inputs). Utilizing a specialized attention block, an LTMI layer matches the representational power of a standard Transformer extension while utilizing less than one-tenth of its parameters, as validated on the VisDial dataset. Finally, we study interactive instruction-following for embodied AI using the ALFRED dataset. We propose a framework featuring a two-stage instruction interpretation: it first decodes language directives independently of visual context to predict a tentative action-object sequence, which is then fused with visual features for final execution. Using multiple egocentric views and hierarchical attention, our method accurately localizes objects and achieves a state-of-the-art unseen success rate of 8.37%.

==> mathdefs.tex <==
%%% mathdefs.tex
%


% Taken from Adam Lupu-Sax ....................................................
%%% derivatives
\newcommand{\deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\derivc}[3]{\left. \frac{d#1}{d#2}\right|_{#3}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdc}[3]{\left. \frac{\partial #1}{\partial #2}\right|_{#3}}

%%% Dirac notation
\newcommand{\bra}[1]{\left\langle #1\right|}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[2]{\left\langle #1 \left|#2\right.\right\rangle}
\newcommand{\braOket}[3]{\left\langle #1\left|#2\right|#3\right\rangle}

% calligraphic letters in math.
\def\cal#1{\mathcal{#1}}


% Taken from M Haggerty ......................................................
\def\avg#1{\left< #1 \right>}
\def\abs#1{\left| #1 \right|}
\def\recip#1{\frac{1}{#1}}
\def\vhat#1{\hat{{\bf #1}}}
\def\smallfrac#1#2{{\textstyle\frac{#1}{#2}}}
\def\smallrecip#1{\smallfrac{1}{#1}}

% SPSmith's definitions ......................................................
\def\spshalf{{1\over{2}}}
\def\Orabi{\Omega_{\rm rabi}}
\def\btt#1{{\tt$\backslash$#1}}




% My own .....................................................................

%%% Equations
\def\schrod{Schroedinger's Equation}
\def\helm{Helmholtz Equation}


%%% Equation environments
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bean{\begin{mathletters}\begin{eqnarray}}
\def\eean{\end{eqnarray}\end{mathletters}}


%%% macros for Feb 2000 PRL
\newcommand{\tbox}[1]{\mbox{\tiny #1}}
\newcommand{\half}{\mbox{\small $\frac{1}{2}$}}
\newcommand{\pit}{\mbox{\small $\frac{\pi}{2}$}}
\newcommand{\sfrac}[1]{\mbox{\small $\frac{1}{#1}$}}
\newcommand{\mbf}[1]{{\mathbf #1}}
% hack to get APS's \text style to work ok:
\def\text{\tbox}

\newcommand{\mV}{{\mathsf{V}}}
\newcommand{\mL}{{\mathsf{L}}}
\newcommand{\mA}{{\mathsf{A}}}
\newcommand{\lB}{\lambda_{\tbox{B}}}  % de Broglie
\newcommand{\ofr}{{(\mbf{r})}}       % (r vec)
\def\ofkr{(k;\mbf{r})}			% (k;r vec)
\def\ofks{(k;\mbf{s})}			% (k;s vec)
\newcommand{\ofs}{{(\mbf{s})}}       % (s vec)
\def\xt{\mbf{x}^{\tbox T}}		% x^T vec

\def\ce{\tilde{C}_{\tbox E}}		% C_E
\def\cew{\tilde{C}_{\tbox E}(\omega)}		% C_E(w)
\def\ceqmw{\tilde{C}^{\tbox{qm}}_{\tbox E}(\omega)}	% C^qm_E(w)
\def\cewqm{\tilde{C}^{\tbox{qm}}_{\tbox E}}	% C^qm_E(w) no omega
\def\ceqm{C^{\tbox{qm}}_{\tbox E}}	% C^qm_E no tilde
\def\cw{\tilde{C}(\omega)}		% C(w)
\def\cfw{\tilde{C}_{\cal F}(\omega)}		% C_F(w)

\def\tcl{\tau_{\tbox{cl}}}		% tau cl
\def\tcol{\tau_{\tbox{col}}}		% tau col
\def\terg{t_{\tbox{erg}}}		% t_erg
\def\tbl{\tau_{\tbox{bl}}}		% tau bl
\def\theis{t_{\tbox{H}}}		% t_Heis

\def\area{\mathsf{A}_D}			% piston effective area A_D 
\def\ve{\nu_{\tbox{E}}}			% nu_E, noise intensity
\def\vewna{\nu_E^{\tbox{WNA}}}		% nu_E for WNA

\def\dxcqm{\delta x^{\tbox{qm}}_{\tbox c}}	% x to mix levels.

%% operators
\newcommand{\rop}{\hat{\mbf{r}}}	% vector valued operators
\newcommand{\pop}{\hat{\mbf{p}}}


%%% Integrals
\newcommand{\sint}{\oint \! d\mbf{s} \,} % surface int
\def\gint{\oint_\Gamma \!\! d\mbf{s} \,} % surface int over Gamma.
\newcommand{\lint}{\oint \! ds \,}	% d=2
\def\infint{\int_{-\infty}^{\infty} \!\!}	% infinite integral
\def\dn{\partial_n}				% d_n
\def\aswapb{a^*\!{\leftrightarrow}b}		% a* <-> b
\def\eps{\varepsilon}				% eps

%%% Dissipation.
\def\dhdxt{\partial {\cal H} / \partial x}
\def\dhdx{\pd{\cal H}{x}}
\def\dhdxnm{\left( \pd{\cal H}{x} \right)_{\!nm}}
\def\dhdxnmsq{\left| \left( \pd{\cal H}{x} \right)_{\!nm} \right| ^2}

%%% vergini
\def\bcs{\stackrel{\tbox{BCs}}{\longrightarrow}}	% apply BCs




%%% DIEL atom project.
\def\wx{\omega_x}
\def\wy{\omega_y}
\newcommand{\ofro}{({\bf r_0})}
\def\Eb{E_{\rm blue,rms}}
\def\Er{E_{\rm red,rms}}
\def\Es2{E_{0,{\rm sat}}^2}
\def\sb{s_{\rm blue}}
\def\sr{s_{\rm red}}

%%% text usefuls
\def\ie{{\it i.e.\ }}
\def\eg{{\it e.g.\ }}
\newcommand{\etal}{{\it et al.\ }}
\newcommand{\ibid}{{\it ibid.\ }}

%%% tables spaces.
\def\gap{\hspace{0.2in}}


%%%%%%%%%%%%%%%%%%%%
%%% mathletters code (from http://www.grad.uiuc.edu/thesis/latexcode.html )
% Modified Alex Barnett 00/9/28 to handle non-arabic \thechapter output
% (ie, now works in Appendices)
% Fails to give correct references in eqnarray (offset by one).
% Still inserts small extra space after equation - unknown reason.
%
%    Original code:
%\newcounter{eqletter}
%\def\mathletters{%
%\setcounter{eqletter}{0}%
%\addtocounter{equation}{1}
%\edef\curreqno{\arabic{equation}}
%\edef\@currentlabel{\theequation}
%\def\theequation{%
%\addtocounter{eqletter}{1}\arabic{chapter}.\curreqno\alph{eqletter}%
%}%
%}
%\def\endmathletters{\setcounter{equation}{\curreqno}}

\newcounter{eqletter}
\def\mathletters{%
\setcounter{eqletter}{0}%
\addtocounter{equation}{1}
\edef\curreqno{\arabic{equation}}
\edef\@currentlabel{\theequation}
\def\theequation{%
\addtocounter{eqletter}{1}\thechapter.\curreqno\alph{eqletter}%
}%
}
\def\endmathletters{\setcounter{equation}{\curreqno}}


%...............................................QPC...................

\newcommand{\bk}{{\bf k}}
\def\kf{k_{\text F}}
\newcommand{\br}{{\bf r}}
\newcommand{\TL}{{\text{(L)}}}
\newcommand{\TR}{{\text{(R)}}}
\newcommand{\TLR}{{\text{L,R}}}
\newcommand{\VSD}{V_{\text{SD}}}
\newcommand{\GT}{\Gamma_{\text{T}}}
\newcommand{\DEL}{\mbox{\boldmath $\nabla$}}
\def\lf{\lambda_{\text F}}
\def\st{\sigma_{\text T}}
\def\stlr{\sigma_{\text T}^{\text{L$\rightarrow$R}}}
\def\strl{\sigma_{\text T}^{\text{R$\rightarrow$L}}}
\def\aeff{a_{\text{eff}}}
\def\aaeff{A_{\text{eff}}}
\def\gat{G_{\text{atom}}}
\newcommand{\LB}{Landauer-B\"{u}ttiker}

% .............. NOTES ..................
% To force linebreak when get overfull hbox from equation in paragraph
% test, use \linebreak (which makes it justify the line it broke).
% Contrast \\ or \newline which leave empty space.
%
%

